RF-Annotate: Automatic RF-Supervised Image Annotation of Common Objects in Context

Wireless tags are increasingly used to track and identify common items of interest such as retail goods, food, medicine, clothing, books, documents, keys, equipment, and more. At the same time, there is a need for labelled visual data featuring such items for the purpose of training object detection and recognition models for robots operating in homes, warehouses, stores, libraries, pharmacies, and so on. In this paper, we ask: can we leverage the tracking and identification capabilities of such tags as a basis for a large-scale automatic image annotation system for robotic perception tasks? We present RF-Annotate, a pipeline for autonomous pixel-wise image annotation which enables robots to collect labelled visual data of objects of interest as they encounter them within their environment. Our pipeline uses unmodified commodity RFID readers and RGB-D cameras, and exploits arbitrary small-scale motions afforded by mobile robotic platforms to spatially map RFIDs to corresponding objects in the scene. Our only assumption is that the objects of interest within the environment are pre-tagged with inexpensive battery-free RFIDs costing 3-15 cents each. We demonstrate the efficacy of our pipeline on several RGB-D sequences of tabletop scenes featuring common objects in a variety of indoor environments.

==> approach.tex <==
\section{Approach}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/pipeline2}
    \caption{\textbf{Pipeline Overview.} PhaseFusion consumes a sequence of synchronously captured RGB-D images, camera poses, and tag readings of a scene. It registers novel instances in a world frame and generates spatial profiles to each instance. It then matches tag responses to instances by bipartite matching on the set of detected instances with the set of detected tags. }\vspace{-0.15in}
    \label{fig:pipeline}
\end{figure*}

In this section, we describe the main components of the our pipeline as outlined in Fig. \ref{fig:pipeline} following the instance segmentation stage, and how each component addresses the issues in the previous section. We assume the set of depth camera images $\{\bI_t\}$, camera poses $\{\bC_t\}$, and tag readings $\{\theta_t\}$ are synchronized with $t \in \{0,\ldots,T-1\}$.

\subsection{Instance Registration}

We take the sequence of instance-labelled depth images $\{\bI_t\}$ and attempt to register the instances into a global frame of reference using the known camera poses $\{\bC_t\}$. First, we transform each depth image $\bI_t$ into a point cloud $\bP_t$ by backprojecting using the known camera intrinsics $\bK$. We then align each point cloud $\bP_t$ into the global reference frame using its corresponding camera pose $\bC_t$. We call the union of these point clouds as the scene $\bG$.

At this stage, $\bG$ still unusable, as the same instances in the scene are not assigned globally consistent instance numbers from the segmentation network. Specifically, the segmentation network labels each instance in each image $\bI_t$ with a number ranging from $[1,N)$, where $N$ is the number of detected instances in the image, but such labels are not consistent across time. To rectify this issue, we must draw correspondences between instances as they appear in different frames.

We accomplish this task by leveraging the well-known point cloud distance metric known as the Chamfer distance. We process the point clouds $\{\bP_t\}$ in order, maintaining a list of instance candidates $\hat{\bX}$. Suppose we are processing $\bP_t$. We extract all the instances in $\bP_t$ and consider their Chamfer distance to the instances within $\hat{\bX}$. If the distance to an instance candidate is under a certain threshold, we consider it a match and update the corresponding instance candidate in $\hat{\bX}$ accordingly. Otherwise, we have found a new instance candidate and append that to $\hat{\bX}$.

To obtain the final list of instances $\bX$, we prune instance candidates from $\hat{\bX}$ which appear in less than a certain fraction of the frames. This is done in order to get rid of spurious instances in the output of the segmentation network induced by depth camera noise.

\subsection{Spatial Profile Generation}

We take the set of instances $\bX$ and generate a set of spatial profiles $\bS_\bX = \{ s_x(t) \mid x \in \bX\}$ for each instance using $\{\bC_t\}$ and a small transform to account for the offset between the tag reader and the depth camera. Each $s_x \in \reals^T$ is a vector describing the variation in distance from the center of the tag reader antenna to the center of the instance point cloud of $x$ in meters. We convert this into a set of differential spatial profiles for each instance $\Delta \bS_\bX$ by taking the difference between consecutive distance values in each $s_x$.

We repeat a similar process for the set of tags $\bY$. Specifically, the tag reader gives us a set of phase profiles of each tag in the scene $\theta_\bY = \{\theta_y(t) \mid y \in \bY\}$. Each $\theta_y \in \reals^T$ is obtained by unwrapping the phase values in the range $[0,180)$. We convert phase changes in consecutive phase readings using the formula \begin{equation} \Delta s = \frac{c}{2\lambda} \cdot \frac{\Delta\theta}{360}\end{equation}, where $c$ is the speed of light and $\lambda$ corresponds to the tag reader wavelength. This allows us to obtain the differential spatial profiles for the tags $\Delta \bS_\bY$.

We note that unlike $\Delta \bS_\bX$, $\Delta \bS_\bY$ can have discontinuities as a result of reader orientation sensitivity and propagation effects in the environment meaning that certain tags are not detected at certain moments in time. We deal with these missing values in the next stage. 

Finally, we take advantage of the stability and accuracy of $\Delta \bS_\bX$ to define a weighting function $w(t)$ that quantifies at each moment in time how discriminative the current camera motion is with respect to the instances in $\bX$. In particular, the current camera motion at time $t$ is more discriminative if $\Delta \bS_\bX(t)$ has high variance. We use normalized variance for $w(t)$, i.e. \begin{equation} w(t) = \frac{\Var(\Delta \bS_X(t))}{\max \Var(\Delta \bS_X(t))}\end{equation} where $0/0 = 1$.

\subsection{Similarity Matching}

At this stage, we are given the differential spatial profiles $\Delta \bS_\bX \in \reals^{|\bX| \times T}$ and $\Delta \bS_\bY \in \reals^{|\bY| \times T}$. Our goal is to determine the most fitting assignment $\bM = \{(x,y) \mid x \in \bX, y \in \bY\}$ between $\bX$ and $\bY$, which corresponds to a maximum weight bipartite matching problem. 

To create the cost matrix, we need a metric $r(\Delta s_x, \Delta s_y)$ that judges the similarity of $x$ and $y$. We opt to use a reward rather than a loss function as this allows us to trivially deal with missing values in $s_y$. We define it as
\begin{equation}
    r(\Delta s_x, \Delta s_y) = \sum_{t=0}^{T-1} w(t) \biggl(1.0 - \min \biggl(1.0, \frac{|\Delta s_x(t) - \Delta s_y(t)|}{F}\biggr)\biggr)
\end{equation}
where $F$ is an appropriately chosen scaling factor. After constructing the cost matrix, we compute $\bM$ using the Hungarian algorithm and update $\bG$ accordingly.

\subsection{Label Reprojection}

Finally, to get the output image labels for an input image $\bI_t$, we simply backproject from $\bG$ using the known camera intrinsics $\bK$ and camera extrinsics $\bC_t$. Specifically, we compare each instance in $\bP_t$ with each instance in $\bG$ using the Chamfer distance, and assign the label corresponding to the best matching instance in $\bG$ before finally projecting $\bP_t$ back into the labelled image $\bI_t$.

==> intro-1.tex <==
\section{Introduction}

Availability of large datasets such as ImageNet~\cite{deng_imagenet_2009}, Pascal VOC~\cite{everingham_pascal_2010}, and MS COCO~\cite{lin_microsoft_2014} is crucial for the success of deep learning in perceptual tasks such as object detection and semantic segmentation. Although standard within the computer vision community, such static datasets are ill-suited for the unique challenges of robotic vision broadly due to the effects of \textit{distributional shift}. Firstly, such datasets typically carry the implicit assumption of a static distribution over a fixed set of categories of interest. In contrast, robots continually operating under \textit{open-set} conditions \cite{sunderhauf_limits_2018} in unstructured and non-stationary environments will invariably encounter novel objects of interest, meaning the categories of interest as well as their relative frequencies are not static. Secondly, such datasets usually feature an inherent bias as they consist of well-curated and highly photogenic Internet images which are not representative of the more mundane and realistic images that a robot is likely to experience under normal and possibly sub-standard operating conditions. ObjectNet \cite{barbu_objectnet_2019} found that state-of-the-art models trained on ImageNet suffer a performance drop of 40--45\% when controls for illumination, occlusion, background, orientation, and viewpoint are introduced, which limits their applicability to many practical settings. An alternative approach is to use simulation to generate synthetic datasets that are more finely controlled, but this paradigm suffers from the well-known domain gap between simulation and reality \cite{gupta_robot_2018}\cite{fang_graspnet-1billion_2020}. 

{\color{red}
Hence, the effectiveness of data-driven approaches in robotic perception is still largely limited by the availability and diversity of high quality real world data. This has culminated in a spate of manually collected and labelled datasets such as YCB \cite{calli_benchmarking_2015}, CORe50 \cite{lomonaco_core50_2017}, ARID \cite{loghmani_recognizing_2018}, OCID \cite{suchi_easylabel_2019} and OpenLORIS-Object\cite{she_openloris-object_2020}, and in a wider sense the creation of an entire image annotation industry \cite{data_annotation}\cite{tesla}. Yet, judging from developments in the autonomous driving space, it is unlikely the amount of data required by deep-learning based methods can be met by conventional labor-intensive manual image annotation pipelines alone.}

\iffalse
{\color{red}
Hence, the effectiveness of data-driven approaches to robotic perception is still largely limited by the availability and diversity of high quality real world data \cite{gupta_robot_2018}\cite{song_grasping_2020}\cite{fang_graspnet-1billion_2020}. To address this, there has been a spate of manually collected datasets such as YCB \cite{calli_benchmarking_2015}, CORe50 \cite{lomonaco_core50_2017}, ARID \cite{loghmani_recognizing_2018}, OCID \cite{suchi_easylabel_2019} and OpenLORIS-Object\cite{she_openloris-object_2020}. In a wider context, this also culminated in the growth of an entire data annotation industry \cite{data_annotation}. Yet, judging from developments in the autonomous driving space, it is unlikely the amount of data required by deep-learning based methods can be met by conventional labor-intensive manual image annotation pipelines alone \cite{tesla}.}
\fi

{\color{red}
Recent work has shown great promise in using robots to autonomously collect real world data for the task of vision-based robotic grasping via self-supervised annotation of successful grasp attempts \cite{pinto_supersizing_2015}\cite{kulic_learning_2017}\cite{gupta_robot_2018}. Hence, we ask: \textit{to what extent can we enable robots to autonomously collect real world data for perceptual tasks such as object detection and semantic segmentation?} We note that automating dense pixelwise image annotation is a far more difficult task than automating successful grasp annotation. Whereas a robot can annotate whether an attempted grasp was successful by simply reading the force sensor readings at its gripper, annotating images for visual recognition tasks such as object detection and segmentation is far more difficult as ambiguities in semantic categories as well as object boundaries in images can confuse even humans. On the other hand, the potential upside in being able to perform such a task is greater, as pixelwise annotation of images with a large variety of possible categories is a far more dense and diverse form of supervision than binary success-or-failure grasp annotations.}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/rf-annotate}
    \caption{Scene containing multiple RFID-tagged objects replying simultaneously to an RFID reader's query. RF-Annotate exploits channel variations to each RFID resulting from arbitrary small-scale robotic motions to match each object instance with the correct RFID response, and thus semantic label.}\vspace{-0.05in}
    \label{fig:intro}
\end{figure}

{\color{red}
Fortunately, parallel developments in the internet-of-things space has yielded the ability to track goods of interest using various technologies such as battery-free passive RFIDs \cite{wang_dude_2013}, BLE trackers such as Tile \cite{tile}, or UWB tags such as Apple's AirTag \cite{airtag} and Samsung's SmartTag+ \cite{smarttag}. Beyond merely locating objects of interest, such tags also allow for the identification and querying of objects and their properties as they can carry either standardized and publicly indexable identification numbers or user-given names, leading to the potential for a very large and rich ontology of possible labels. Hence, the question becomes: \textit{can we leverage the capabilities of such tags for fully automatic image annotation of common objects in robotic environments?} 

Exploring this possibility in the context of passive RFID tags, we present RF-Annotate, the first automatic pipeline that allows robots to generate their own pixelwise annotated RGB-D images of RFID-tagged common objects in robotic environments without continuous human supervision. It only requires that objects of interest within the environment are pre-tagged with passive RFIDs, which embed relevant information for each object such as object class and unique serial numbers in the form of a standardized EPC code \cite{epc}.} To summarize, we make the following contributions.
\begin{itemize}[leftmargin=*]
    \item We present RF-Annotate, the first RF-based pipeline for fully autonomous dense pixelwise image annotation that enables scalable real world data gathering for visual recognition and segmentation tasks in robotic environments without continuous human intervention.
    \item We empirically observe the detrimental effects of hardware \& environmental noise and missing values within the readings of both the RGB-D camera and the RFID reader in unstructured real world environments, and propose a strategy for filtering out noise and missing values by fusing information from multiple views and readings of a scene.
    \item We demonstrate the effectiveness of the pipeline on several real world RGB-D sequences of RFID-tagged scenes by comparing the results to manually labelled images of the same scene.
\end{itemize}

\iffalse
\name's design has three key components:

\begin{itemize}[leftmargin=*]
\item First, it leverages an RFID reader to query the set of RFID tags present in the environment. RFIDs operate via UHF radio waves at a range of few feet, and single query can reveal the set of objects present in a scene even through occlusions. Note however, that a reader on its own cannot localize the source of each reply.

\item Secondly, it leverages an \textit{unseen} object instance segmentation network pre-trained on synthetic CAD models \cite{xiang_learning_2021} as a geometric prior to propose novel (unlabelled) object instances within the robot's environment. This step bypasses the need for per-class predetermined CAD models and active human input to map these models to the respective objects in the visual scene as in LabelFusion \cite{marion_labelfusion_2017}. Although trained on non-photorealistic synthetic data, the instance segmentation network can generalize to reality through the depth channel as the domain gap in the depth channel is far less than that of color due to its invariance to differing textures and lighting conditions.

{\color{red}
\item Finally, given the set of unlabelled object instances and RFID tags, we design a signal processing framework that maps each object instance to its corresponding RFID tag (and hence, an accurate label). Our insight is that the tag and the object have correlated motion with respect to the robot. To extract such spatial information, we leverage the ability of the robot to move the data capture apparatus within the environment to gain more information about the scene as necessary. %In particular, the pipeline takes a spatio-temporally correlated sequence of synchronously captured RGB-D images and RFID tag responses of the scene from various angles. This is necessary as information from multiple views of the scene is necessary to accomplish the expected outcome.
}
\end{itemize}

{\color{red}
Finally, we note that RF-Annotate focuses on automating dense pixelwise image annotation, which is a far more difficult task than automating binary grasp annotation \cite{pinto_supersizing_2015} \cite{gupta_robot_2018}. Whereas a robot can annotate whether an attempted grasp was successful by simply reading the force sensor readings at its gripper, annotating images for visual recognition tasks such as object detection and segmentation is far more difficult as ambiguities in semantic categories as well as object boundaries in images can confuse even humans. On the other hand, the potential upside in being able to perform such a task is more rewarding, as pixelwise annotation of images with a rich ontology of categories as afforded by publicly searchable EPC codes is a far more dense form of supervision than mere binary grasp annotation.}



To summarize, we make the following contributions.
\begin{itemize}[leftmargin=*]
    \item We present RF-Annotate, the first RF-based pipeline for fully autonomous dense pixelwise image annotation that enables scalable real world data gathering for visual recognition and segmentation tasks in robotic environments without continuous human intervention.
    \item We empirically observe the detrimental effects of hardware \& environmental noise and missing values within the readings of both the RGB-D camera and the RFID reader in unstructured real world environments, and propose a strategy for filtering out noise and missing values by fusing information from multiple views and readings of a scene.
    \item We demonstrate the effectiveness of the pipeline on several real world RGB-D sequences of RFID-tagged scenes by comparing the results to manually labelled images of the same scene.
\end{itemize}

\fi

==> intro.tex <==
\section{INTRODUCTION}

Availability of large-scale high quality datasets, such as ImageNet~\cite{deng_imagenet_2009}, Pascal VOC~\cite{everingham_pascal_2010}, and MS COCO~\cite{lin_microsoft_2014} is crucial for the success of deep learning in perceptual tasks. Although considered standard within the computer vision community, such static datasets are ill-suited for the unique challenges of robotic vision broadly due to the effects of \textit{distributional shift}. Firstly, such datasets typically carry the implicit assumption of a static distribution over a fixed set of categories of interest. In contrast, robots continually operating under \textit{open-set} conditions \cite{sunderhauf_limits_2018} in unstructured and non-stationary environments will invariably encounter novel objects of interest, meaning the categories of interest as well as their relative frequencies are not static. Secondly, such datasets usually feature an inherent bias as they consist of well-curated and highly photogenic Internet images which are not representative of the more mundane and realistic images that a robot is likely to experience under normal and possibly sub-standard operating conditions. ObjectNet \cite{barbu_objectnet_2019} found that state-of-the-art models trained on ImageNet suffer a performance drop of 40--45\% when controls for illumination, occlusion, background, orientation, and viewpoint are introduced, which limits their applicability to many practical settings.
\iffalse Hence, additional data from the robot's operating environment collected at deployment time is becomes invaluable for addressing this issue.\fi One alternative approach is to use simulation to generate synthetic datasets that are more finely controlled. However, this paradigm suffers from a similar issue called the Sim2Real problem as models trained in simulation typically suffer when deployed in the real world due to the domain gap between simulation and reality.

In this paper, we ask: \textit{how can we enable robots to autonomously collect real annotated data in previously unseen environments for visual recognition tasks?} This question is important because: (a) the effectiveness of data-driven approaches to robotic perception is still largely limited in the real world by the availability of high quality realistic data, (b) manually annotating objects in every new environment is a labor-intensive task that needs to be repeated as new objects are introduced. Past work such as \cite{gupta_robot_2018} and \cite{song_grasping_2020} has shown that data collected from real environments which strongly resemble the deployment scenario is vital to data-driven approaches for the task of visual grasping. To mitigate the absence of realistic data for visual recognition tasks, there have been several efforts to collect \textit{manually-labelled} datasets in robotic environments: YCB \cite{calli_benchmarking_2015}, CORe50 \cite{lomonaco_core50_2017}, ARID \cite{loghmani_recognizing_2018}, OCID \cite{suchi_easylabel_2019} and OpenLORIS-Object\cite{she_openloris-object_2020}. 

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{figs/intro_alt}
    \caption{RF-Annotate leverages RFIDs as real world ground truth labels, allowing robots to opportunistically collect multi-view pixelwise annotated images of cluttered real world tabletop scenes of objects without continuous human supervision.}\vspace{-0.05in}
    \label{fig:intro}
\end{figure}

We present \name, the first fully autonomous pipeline that allows robots to generate their own pixelwise annotated RGB-D images of RFID-tagged YCB-like objects in indoor robotic environments such as warehouses, offices, and smart homes without continuous human supervision. It only requires that humans tag objects of interest within the environment with RFIDs prior to the robot's deployment. \name\ leverages three key ideas.

\begin{itemize}[leftmargin=*]

\item First, it leverages inexpensive battery-free RFIDs as real world ground truth labels, and builds off previous work on RFID localization and tracking. RFIDs are suited for this purpose as they are capable of associating each object instance in a supply chain with a globally unique serial number and object class as regulated by a universal standard \cite{noauthor_tag_nodate}. The standard consequently makes consistent and scalable centralized data collection of the same object class across different geographical environments and deployment scenarios trivial. Furthermore, it allows for language grounding of the visual representation of such objects, which is useful for upstream natural language related tasks.

\item Secondly, it bypasses the need for predetermined CAD models or shapes as in LabelFusion \cite{marion_labelfusion_2017} by instead leveraging an unseen object instance segmentation network pre-trained on synthetic CAD models \cite{xie_unseen_2020} as a geometric prior to propose novel object instances within the robot's environment. As long as depth information is available, such a network can generalize to reality as the domain gap in the depth channel is far less than that of color due to it being invariant to differing textures and lighting conditions.

\item Thirdly, it leverages the paradigm of \textit{active perception}, where we assume the robot can move the data capture apparatus within the environment to gain more information about the scene as necessary. In particular, the pipeline takes a spatio-temporally correlated sequence of synchronously captured RGB-D images and RFID tag responses of the scene from various angles. This is necessary as information from multiple views of the scene is necessary to accomplish the expected outcome.
\end{itemize}

We note that RF-Annotate focuses on the general task of robotic perception as opposed to tasks like vision-based robotic grasping, where a robot can tell whether an attempted grasp was successful without human intervention, allowing robots to collect data for the task autonomously \cite{pinto_supersizing_2015}\cite{gupta_robot_2018}. However, annotating images for visual recognition tasks like object detection and segmentation is far more difficult as ambiguities in images and semantic categories can confuse even humans. This limits the inherent scalability of conventional methods of collecting data for visual recognition tasks. 

To summarize, we make the following contributions.
\begin{itemize}[leftmargin=*]
    \item We present RF-Annotate, the first RF-based pipeline for fully autonomous dense pixelwise image annotation that enables scalable real world data gathering for visual recognition tasks in robotic environments without continuous human intervention.
    \item We empirically observe the detrimental effects of noise and missing values within the readings of both the RGB-D camera and the RFID reader in unstructured real world environments, and propose a strategy for filtering out noise and missing values by fusing information from multiple views and readings of a scene.
    \item We demonstrate the effectiveness of the pipeline on several real world RGB-D sequences of RFID-tagged scenes by comparing the results to manually labelled images of the same scene.
    \iffalse
    \item We demonstrate the utility of the data generated by the pipeline by fine-tuning pre-trained models from the Internet and measuring the corresponding performance increase in the deployed environment.
    \fi
\end{itemize}




==> problem.tex <==
\section{Problem Statement}

We are given a spatio-temporally correlated sequence of synchronously captured RGB-D images, tag readings, and camera poses of a static cluttered tabletop scene of RFID-tagged objects as captured using the setup in Fig. \ref{fig:experiments}. Our goal is to perform pixelwise annotation of each object with the label of its corresponding RFID for images in the sequence.

In brief, this entails the following. First, we discover novel instances within the scene by segmenting them using a pre-trained model on each individual RGB-D image. We use UCN \cite{xie_unseen_2020} for this purpose, although any network capable of generating instance proposals from RGB-D images can be used. Second, we process the tag readings of the scene in order to associate the RFID responses to the appropriate novel object instances as obtained in the first stage in a bipartite matching problem. This produces a set of labelled instances within the scene. Finally, we backproject the labelled instances into each image in the sequence using the camera parameters in order to obtain the final set of annotated output images.

Although such a task seems straightforward, there are several key challenges to consider. Since the data is captured in the real world with imperfect low-cost commodity hardware, the effects of noise and missing values within the sensor readings are highly prominent. We confirm this after experimenting with various combinations of hardware in various unstructured environments. We empirically observe the following effects:
\begin{itemize}[leftmargin=*]
    \item \textbf{Depth Camera Noise.} Most commodity indoor depth cameras such as the Kinect or RealSense operate using depth-from-disparity from a IR pattern projected onto scene. However, it is common to observe missing depth values due to various effects like shadowing and occlusions that occur in real scenes. Furthermore, the depth values slightly vary over time even when held fixed pointing towards a static scene due to temporal noise effects. These factors affect both the quality and consistency of output of the segmentation network as it is trained on perfect synthetic depth images generated in simulation. It is not uncommon, for example, to observe spurious instances which are detected intermittently even without moving the camera or any objects within the scene.
    \item \textbf{Tag Reader Noise.} The propagation of a signal from a tag reader to an RFID tag is affected by hardware as well as environmental factors. On the hardware side, one limitation of commodity RFID readers is that they only report channel phase values within the range of $[0,180)$ culminating in a $180$ degree phase ambiguity. Perhaps the most prominent environmental factor is multipath propagation, which occurs when the signal reflects off of various things in the environment, creating multiple copies of itself that arrive at the reader and interfere. Both environmental and hardware related factors can cause the channel to vary temporally when everything else is held fixed. Furthermore, RFIDs are orientation sensitive, meaning they are easier to read from certain angles than others. This means the channel readings to each individual RFID is scarcely continuous as the data collection apparatus is moved around the scene in an unstructured manner.
    \item \textbf{Non-discriminative Motions.} We do not observe significant noise in the readings of the visual-inertial tracking module under normal operating conditions. However, the camera trajectory can contribute noise towards the results of the pipeline indirectly through redundant motions that do not act to significantly distinguish the instances and tags within the scene. Generally speaking, moving towards or away from the scene contributes less new information than sideways motion. If a trajectory contains too many such redundant motions in comparison to informative motions, the pipeline may fail.
\end{itemize}

\iffalse
Hence, our goal is to create a pipeline that is robust to such imperfections in these sensor readings. 
\fi
\iffalse
Clearly, making such a scheme practical entails devising techniques to handle such imperfections in these sensor readings. In particular, we desire that the pipeline is able to continually fuse information of the scene from multiple viewing angles and improve its accuracy with increasing amounts of evidence.
\fi

